OAG-Bench: A Human-Curated Benchmark for Academic Graph Mining

With the rapid proliferation of scientific literature, versatile academic knowledge services increasingly rely on comprehensive academic graph mining. Despite the availability of public academic graphs, benchmarks, and datasets, these resources often fall short in multi-aspect and fine-grained annotations, are constrained to specific task types and domains, or lack underlying real academic graphs. In this paper, we present OAG-Bench, a comprehensive, multi-aspect, and fine-grained human-curated benchmark based on the Open Academic Graph (OAG). OAG-Bench covers 10 tasks, 20 datasets, 70+ baselines, and 120+ experimental results to date. We propose new data annotation strategies for certain tasks and offer a suite of data pre-processing codes, algorithm implementations, and standardized evaluation protocols to facilitate academic graph mining. Extensive experiments reveal that even advanced algorithms like large language models (LLMs) encounter difficulties in addressing key challenges in certain tasks, such as paper source tracing and scholar profiling. We also introduce the Open Academic Graph Challenge (OAG-Challenge) to encourage community input and sharing. We envisage that OAG-Bench can serve as a common ground for the community to evaluate and compare algorithms in academic graph mining, thereby accelerating algorithm development and advancement in this field. OAG-Bench is accessible at https://www.aminer.cn/data/.

==> chapter/entity-alignment.tex <==


\subsection{Entity Alignment}

Entity alignment aims to match the same entities across various data sources.
% This problem has been extensively studied for decades but still remains challenging
It is a long-studied yet challenging issue 
due to missing, ambiguous, and heterogeneous entity attributes.
This subsection provides $3$ datasets corresponding to $3$ different types of entities,
including venues, affiliations, and authors.
The problem definition of entity alignment is defined below.

\theoremstyle{problem}
\begin{problem}{\bf Entity Alignment.} 
    Given two entity sets $E_1$ and $E_2$,
    the goal is to generate entity alignments 
    $L = \{(e_1, e_2) | e_1 \in E_1, e_2 \in E_2\}$ such that 
    $e_1$ and $e_2$ actually refer to the same real-world entity.
\end{problem}

% Entity alignment consists of $3$ subtasks: 
% venue alignment, affiliation alignment, and author alignment.
% Each subtask corresponds to a dataset.
% The three datasets are detailed below.

\vpara{Datasets.}
(1) \textbf{Venue}~\cite{zhang2019oag}:
We've created a challenging venue alignment dataset 
by excluding direct full-name or abbreviation matches.
It consists of $1{\small,}200$ manual annotations, 
including $510$ positive and $690$ negative pairs. 
The dataset is randomly split into training, validation, and test sets at a $4: 1: 1$ ratio.
(2) \textbf{\textit{Affiliation}}:
This dataset comprises $5{\small,}000$ affiliation pairs,
each linked to a Wikipedia page.
Positive pairs are created by selecting former names or aliases from Wikipedia entries, while negative pairs are generated by searching for the current entity in the MAG affiliation set and selecting the second-ranked affiliation. 
% The dataset is split randomly into training, validation, and test sets ($3: 1: 1$ ratio).
The dataset is randomly partitioned into training, validation, and test sets, adhering to a ratio of $3:1:1$, respectively.
(3) \textbf{\textit{Author}}:
This dataset includes \num{10000} human-annotated author alignment pairs between AMiner and DBLP.
% The dataset is split randomly into training, validation, and test sets ($8 :1 :1$ ratio). 
The dataset is randomly divided into training, validation, and test sets, following an $8:1:1$ ratio.
It also provides authors' published papers and detailed author properties.

\hide{
\begin{itemize}[leftmargin=*]
    \item \textbf{Venue alignment dataset:}
    A difficult venue alignment dataset is constructed,
    where venue alignment pairs that can be directly matched by 
    full name or abbreviation are removed.
    This dataset contains \num{1200} manually annotated venue alignment pairs,
    of which $510$ are positive pairs and $690$ are negative pairs.
    The dataset is randomly divided so that 
    the ratio of training set, validation set, and test set is $4: 1: 1$.
    \item \textbf{Affiliation alignment dataset:}
    This dataset includes \num{5000} affiliation pairs.
    Based on the affiliation set in Microsoft Academic,
    each affiliation is associated with a Wikipedia page.
    The method of constructing a positive pair is to select the 
    former name or alias of the affiliation in the Wikipedia entry.
    The method of constructing a negative pair is to search for 
    the current entity via Elastic Search\footnote{\url{https://www.elastic.co/}} 
    in the affiliation set of Microsoft Academic,
    and select the second-ranked affiliation as a negative example
    (the first-ranked affiliation is the current entity itself).
    The ratio of positive and negative pairs is $1: 1$.
    The dataset is randomly divided so that the ratio of 
    training set, validation set, and test set is $3: 1: 1$.
    \item \textbf{Author alignment dataset:}
    This dataset contains \num{10000} human-annotated author alignment pairs between AMiner and DBLP.
    In order to construct hard negative author pairs,
    the method of constructing a negative pair is:
    if the author has an author with the same name in DBLP,
    then select a different author with the same name as a negative pair;
    otherwise, the most frequent collaborators of the aligned author in DBLP
    is taken as a negative pair.
    The ratio of positive and negative pairs is $1: 1$.
    Furthermore, the ratio of training set, validation set, and test set is $8: 1: 1$, and the published papers and detailed properties of each author are also provided.
\end{itemize}
}

\vpara{Evaluation Metrics.}
Entity alignment is a binary classification problem.
% The evaluation metrics are precision, recall, F1, and AUC.
% We report F1 and AUC here.
We take F1 and AUC as the evaluation metric.


% \vpara{Comparsion Methods.}
% We adopt traditional machine learning methods (such as SVM)
% and a variety of neural network-based matching methods for comparison.
\vpara{Baselines.}
We compare different types of matching methods:
(1) traditional machine learning methods (\textbf{SVM})
using Jaccard index and TF-IDF similarity as input features;
(2) shallow neural network-based matching methods
including CNN-based matching model (\textbf{\modeloagcnn})~\cite{zhang2019oag}
and RNN-based matching model (\textbf{\modeloaglstm})~\cite{zhang2019oag};
(3) matching models based on pre-trained models (\textbf{Ditto}~\cite{li2020deep}
with pre-trained models BERT~\cite{devlin2019bert}, ALBERT~\cite{lan2019albert}, 
RoBERTa~\cite{liu2019roberta}, DeBERTa~\cite{he2022debertav3}, 
LaBSE~\cite{feng2022language}, and GLM~\cite{du2022glm}).

\hide{
\begin{itemize}[leftmargin=*]
    \item \textbf{SVM:} 
    For venue alignment and affiliation alignment,
    Jaccard index of text pairs and 
    the cosine similarity calculated by TF-IDF are selected as input features.
    For author alignment,
    the Jaccard index of the paper sets of two authors
    and the Jaccard index of two authors' venue sets are selected as input features.
    \item \textbf{\modeloagcnn~\cite{zhang2019oag}:}
    For each candidate pair,
    this method first constructs word-level similarity matrices for each attribute,
    and then uses CNN to map these matrices into similarity vectors.
    Then, the similarity vectors of different attributes are concatenated 
    and passed to the fully connected layers for classification.
    For venue and affiliation entities,
    we use the entity's integral sequence and keyword sequence as entity attributes.
    For author entities, we use the venue ID list and paper ID list
    associated with the authors as entity attributes.
    \item \textbf{\modeloaglstm~\cite{zhang2019oag}:}
    This method treats each entity attribute as a sequence of words.
    The content of each attribute is encoded as a vector by LSTM.
    For each candidate pair, the vectors of the same attributes are merged
    (such as concatenation, subtraction, etc.) into a similarity vector,
    and then passed to the fully-connected layers to predict the matching label.
    This method uses the same entity attributes as \modeloagcnn for alignment.
    \item \textbf{\modeloaggat~\cite{zhang2019oag}:}
    This method is used for author alignment.
    This method constructs a subgraph for each candidate pair.
    Two subgraphs can be connected by aligned entities.
    Then heterogeneous graph attention network is used to encode the subgraph
    and predict the alignment label.
    Specifically, each author's papers, published venues, and coauthors
    are used as nodes in the subgraph to construct a two-hop subgraph.
    Also, entities (venues or papers) can be merged between AMiner and DBLP,
    since the two types of entities are less ambiguous.
    In addition, this method incorporates the features used in the 
    aforementioned SVM to enhance the matching performance.
\end{itemize}
}

\hide{

\begin{table}[t]
	\centering
	\newcolumntype{?}{!{\vrule width 1pt}}
	\caption{
        Alignment results of different types of entities ($\%$)
	}
	\label{tb:entity-matching}
	\begin{tabular}{  c | p{1cm} <{\centering}? p{1cm} <{\centering}| p{1cm}<{\centering}| p{1cm}<{\centering} | p{1cm}<{\centering}}
		\toprule
		\multicolumn{2}{c?}{Method} & {SVM} & \modeloagcnn  & \modeloaglstm & \modeloaggat \\
		
        \midrule
		\multirow{4}*{Venue} 
	    & Prec.  & 76.67 & 85.78 & 83.88 & -- \\
		~ & Rec. & 89.61 & 81.56 & 86.49 & --\\
        ~ & F1   & 82.63 & 83.46 & \textbf{85.03} & --\\
		~ & AUC  & 91.87 & 94.07 & \textbf{95.33} & --\\

		\midrule
		
		\multirow{4}*{Affiliation} 
	    & Prec.  & 66.11 & 61.23 & 66.18 & -- \\
		~ & Rec. & 73.00 & 79.8 & 69.88 &  --\\
        ~ & F1   & 68.47 & \textbf{69.06} & 67.76 & --\\
		~ & AUC  & 70.93 & 69.12 & \textbf{72.37} & --\\
		\midrule
		
		\multirow{4}*{Author} 
	    & Prec.  & 98.35 & 57.23 & 65.58 & 98.33 \\
		~ & Rec. & 83.20 & 83.00 & 87.44 & 82.36 \\
        ~ & F1   & \textbf{90.14} & 67.72 & 74.80 & 89.62 \\
		~ & AUC  & 93.67 & 66.78 & 77.58 & \textbf{97.32} \\
		\bottomrule
	\end{tabular}
\end{table}

}


\begin{table}[t]
    \newcolumntype{C}{>{\centering\arraybackslash}p{2.2em}}
    \caption{
        \label{tb:entity-matching} Alignment results of different types of entities ($\%$).
    }
    \centering
    \renewcommand\arraystretch{1.0}
    \begin{tabular}{c|@{~ }*{1}{CC|}*{1}CC}
        \toprule[1.2pt]
        &\multicolumn{2}{c|}{Venue}
        &\multicolumn{2}{c}{Affiliation}
    \\
    \cmidrule{2-3} \cmidrule{4-5} 
    {Method}   & {F1} & {AUC} & {F1}  & {AUC}   \\
    \midrule
    SVM & 82.63 & 91.87 & 68.47 & 70.93 \\
    \modeloagcnn & 83.46 & 94.07 & 69.06 & 69.12 \\
    \modeloaglstm & 85.03 & 95.33 & 67.76 & 72.37 \\
    % \midrule
    Ditto-BERT-base & 89.33 & 95.00 & 70.38 & 78.65 \\
    Ditto-ALBERT-base & 88.05 & 96.06 & 61.90 & 70.96 \\
    Ditto-RoBERTa-large & 89.47 & 97.22 & 71.98 & 79.02 \\
    Ditto-DeBERTa-base & \textbf{94.27} & 96.73 & 72.78 & 80.37\\
    Ditto-DeBERTa-large & 89.44 & \textbf{97.94} & \textbf{82.18} & \textbf{89.76} \\
    Ditto-LaBSE & 90.79 & 96.93 & 71.06 & 78.55 \\
    Ditto-GLM-RoBERTa & 78.82 & 93.04 & 61.11 & 67.93 \\
    \bottomrule[1.2pt]
\end{tabular}
\end{table}


\vpara{Experimental Results.}
Table \ref{tb:entity-matching} presents results for various matching models.
% We omit the results of author alignment as corresponding methods are graph-based methods.
% Author alignment results are omitted as they use graph-based methods. 
The methods for author alignment utilize more structural information, 
with corresponding results presented in Section \ref{app:author_alignment}.
% It can be seen that the optimal models for different types of entity-matching tasks are different.
Venue/affiliation alignment is essentially a short text matching task.
% \modeloagcnn and \modeloaglstm achieve good results on both tasks.
% \modeloaglstm slightly outperforms \modeloagcnn in venue matching.
% It shows that both the CNN-based matching model and LSTM-based matching model
% can effectively capture the matching signal of texts
% (such as contextual dependence of words in the sequence).
SVM performs slightly poorer than \modeloagcnn and \modeloaglstm,
% on venue matching and affiliation matching tasks,
% possibly because the SVM features cannot capture word order information.
possibly due to the inability of SVM features to capture word order information.
% For author matching, methods using authors' structure information (SVM and \modeloaggat)
% are significantly better than methods not using structure information (\modeloagcnn and \modeloaglstm).
Conversely, \modeloagcnn and \modeloaglstm can capture the contextual dependence of word sequence.
Overall, the top-performing models on both datasets utilize pre-training, 
indicating the promising potential of pre-trained language models for entity alignment.
Among all methods that employ pre-trained models, 
DeBERTa-large delivers the best performance on two tasks, particularly on affiliation alignment,
indicating that DeBERTa-large effectively encodes additional semantic knowledge beyond affiliations' surface names.
Note that the trends of AUC and F1 in the table are sometimes inconsistent.
% Considering F1 needs to set a threshold, 
Given that F1 requires a threshold setting, 
% it is more reasonable to focus on AUC when AUC and F1 are inconsistent.
AUC is a more reliable metric when discrepancies arise between the two.
% In addition, the highest AUC is $72.37\%$ for affiliation matching,
% and there is still a lot of root for improvement.
% One possible reason is that it is difficult to match the different aliases of affiliations
% only using the affiliation names.
% Thus, more affiliation attributes may need to be incoporated.
% For author matching, more author pairs with ambiguous names will be added
% in the future to increase the difficulty of this task.

